Universal Marginaliser for Deep Amortised Inference for Probabilistic Programs

Probabilistic programming languages (PPLs) are powerful modelling tools which allow to formalise our knowledge about the world and reason about its inherent uncertainty. Inference methods used in PPL can be computationally costly due to significant time burden and/or storage requirements; or they can lack theoretical guarantees of convergence and accuracy when applied to large scale graphical models. To this end, we present the Universal Marginaliser (UM), a novel method for amortised inference, in PPL. We show how combining samples drawn from the original probabilistic program prior with an appropriate augmentation method allows us to train one neural network to approximate any of the corresponding conditional marginal distributions, with any separation into latent and observed variables, and thus amortise the cost of inference. Finally, we benchmark the method on multiple probabilistic programs, in Pyro, with different model structure.

==> Makefile <==
PROJECT=main

bibtex=refs
pdflatex=pdflatex

BIBTEX=$(bibtex) build/$(PROJECT).aux
BUILDTEX=$(pdflatex) \
		 -halt-on-error \
		--output-directory build \
		-aux-directory=build \
		$(PROJECT).tex


all:
	$(BUILDTEX)
	bibtex build/$(PROJECT).aux
	$(BUILDTEX)
	$(BUILDTEX)

clean:
	rm -rf build/*


==> fig/train.tex <==
\begin{figure*}[ht]
\begin{subfigure}{0.4\linewidth}
  \centering
  \begin{tikzpicture}[node distance=1.6cm, scale=0.60, transform shape]
    \node (PGM) [io] {1. Samples from PGM: $S_i\in \{0,1\}^N$.}; 
    \node (mask) [process, below of=PGM] {2. Mask $\textbf{S}$: $M:\{0,1\}\to \{0,1,*\}$,
      $M:$ probabilistic and/or deterministic.}; 
    \node (masked) [io, below of=mask] {3. Input: $S^{masked}_i := M(S_i)\in\{0,1,*\}^N$, Labels: $S_i$}; 
    \draw [arrow] (PGM) -- (mask);  
    \node (train) [process, below of=masked] {4. Neural network with sigmoid output.};
        \draw [arrow] (mask) -- (masked);  
          \node (output) [io, below of=train] {5. Output: Predicted
      Posterior $P(S_i | S^{masked}_i)$}; 
      \draw [arrow] (train) -- (output); \draw [arrow] (masked) -- (train);
    \path [->, red, very thick] (train) edge[loop right] node (CE)
    [right, black] {min. entropy loss} (train) ;
  \end{tikzpicture}
  \caption{\textbf{UM Training:} The process to train a Universal Marginaliser using binary data generated from a Bayesian Network}
  \label{fig:train}
\end{subfigure}
\hfill
\begin{subfigure}{0.4\linewidth}
  \centering
  \begin{tikzpicture}[node distance=1.6cm, scale=0.5, transform shape]
    \node (inp) [io] {Input: $\mathbf{\hat{X}}\in\{0,1,*\}^N$};
    \node (test_data) [io, below of=inp] {NN Input: $\mathbf{\hat{X}} \cup \{X_1,...X_{i-1}\} \in\{0,1,*\}^N$};
    \draw [arrow] (inp) -- (test_data);
          \node (train_output) [process, below of=test_data] {UM (Trained neural network)}; 
    \draw [arrow] (test_data) -- (train_output); 
    \node (sample) [io, below of=train_output] {Output: $q =
      Q(X_i | \mathbf{\hat{X}} \cup \{X_1,...X_{i-1}\})$}; \node (impo) [process, below
    of=sample] {Sample node $X_i$ with $q$ as proposal}; \draw
    [arrow] (sample) -- (impo); 
    \draw [arrow] (train_output) -- (sample); 
    \node (i) [right of=test_data,xshift=4cm] {$i = i+1$}; 
    \node (ce) [right of=sample,xshift=4cm] {node sample $X_i \in \{0,1\}$}; \draw [->, black] (impo) -- (ce) -- (i) -- (test_data) ; 
    \node (full_sample) [io, below of=impo] {Output: One sample from joint $Q(\mathbf{\hat{X}})$}; \draw [arrow] (impo) -- (full_sample); 
      %\node[draw,inner sep=13mm, fit=(test_data) (train_output) (sample) (i) (ce)(impo)] {};
  \end{tikzpicture}
        \caption{\textbf{Inference using UM-IS}: The part in the box is repeated $N$ times, for each node $i$ in topological order}
  \label{fig:inf}
\end{subfigure}
\end{figure*}


==> images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}

